Nutzung von Massespeichern zur Flexibilisierung des Energieverbrauchs: Kosteneffizienter Anlagenbetrieb durch Anpassung an Marktpreise

The increasing share of renewable energy sources and necessitate new concepts for energy flexible operation of industrial production resources. In this paper, we demonstrate the potential of mass storage to increase energy flexibility in industrial operations through the application of optimized operational planning based on market prices. A wastewater treatment plant equipped with decanters and storages is examined to optimally utilize its energy-flexibility. An MILP model was created for energy-flexible production facilities. The resulting operation plan was transmitted to the plant operators and executed over a period of more than 24 hours. The model shows good agreement with real measurements (average errors between 3% to 7%). The results demonstrate significant potential for cost savings of roughly 56% for the investigated time horizon. -- Der zunehmende Anteil erneuerbarer Energien erfordert neue Konzepte zur energieflexiblen Steuerung industrieller Produktionsanlagen. In diesem Beitrag wird demonstriert, wie das Potenzial von Massespeichern zur Steigerung der Energieflexibilit\"at in industriellen Prozessen durch die Anwendung optimierter Betriebsplanung basierend auf Marktpreisen, genutzt werden kann. Es wird eine Abwasseraufbereitungsanlage mit Dekantern und zugeh\"origen Massespeichersystemen betrachtet, um deren Energieflexibilit\"at optimiert zu nutzen. Der resultierende Betriebsplan wurde in einem Assistenzsystem an die Anlagenbetreiber \"ubermittelt und \"uber einen Zeitraum von \"uber 24 Stunden ausgef\"uhrt. Das Modell zeigt eine gute \"Ubereinstimmung mit den realen Messwerten (Fehlern zwischen 3% und 7%). Alle von den Betreibern gesetzten Betriebsziele wurden erreicht, was die Anwendbarkeit des Modells in industriellen Umgebungen best\"atigt. Die Ergebnisse zeigen ein erhebliches Einsparpotenzial von etwa 56% f\"ur den untersuchten Zeitraum.

==> 2relwork.tex <==
\section{Konzepte zur Flexibilisierung des Anlagenbetriebs} \label{sec:relwork}
\noindent In diesem Abschnitt werden Arbeiten analysiert, welche die Flexibilisierung des Betriebs Energie verbrauchender und -erzeugender Anlagen in der realen Anwendung betrachten.

\citet{GFS+22} optimieren den Stromverbrauch einer industriellen Reinigungsmaschine. Obwohl der untersuchte experimentelle Aufbau in einem industriellen Umfeld liegt, wird kein Produkt hergestellt, weshalb der Einfluss von Optimierungsstrategien auf das Produktionsvolumen nicht untersucht werden kann. \todo[inline]{Lasse: wie geht das? wie wird eine Maschine betrieben, stellt aber kein Produkt her? /// Naja, das Produkt in diesem Fall ist halt 'Sauberkeit' Aber wie quantifiziert man das? Eine Reinigungsmaschine macht halt sauber aber stellt kein physisches Produkt her. }

\citet{PCF+19} beschreiben einen experimentellen Aufbau für den optimierten Betrieb von Wärmepumpen mit variabler Leistung, um die Energieflexibilität von Gebäuden zu erhöhen. Ein Testaufbau für auf erneuerbaren Energien basierende Mikronetze wird von \citet{RCS+21} präsentiert. Keiner der beiden Aufbauten ist jedoch darauf ausgelegt, die Erfüllung von Produktionsplänen zu bewerten.

% Ein experimenteller Aufbau eines Wärmespeichersystems für industrielle Anwendungen wird von \citet{SSK+20} präsentiert.  \citet{SSK+20} stellen fest, dass angemessene Optimierungsstrategien benötigt werden, um industrielle Flexibilität zu nutzen, und dass ihr experimenteller Aufbau gut geeignet ist, solche Strategien zu analysieren. 

% ### 1. "Experimental validation of a state-of-the-art model predictive control approach for demand side management with a hot water heat pump" von Baumann et al.

% \citet{BHA+23} untersuchen die  Optimierung des Betriebs von Wärmepumpen. Durch experimentelle Tests wurde gezeigt, dass signifikante Energieeinsparungen und Effizienzsteigerungen im Vergleich zur herkömmlichen Hystereseregelung generiert werden können. Trotz der positiven Ergebnisse wurde die Implementierung in einer kontrollierten Laborumgebung durchgeführt, wobei Herausforderungen bei der Interaktion mit lokalen Controllern und festen Herstellereinstellungen auftraten. Eine weiterführende Anwendung unter realen Betriebsbedingungen wird jedoch nicht beschrieben, um die Ergebnisse umfassend zu validieren.

% %### 3. "A digital twin-based adaptive optimization approach applied to waste heat recovery in green steel production: Development and experimental investigation" von Kasper et al.

% \citet{KSB+24} implementieren einen Optimierungsansatz zur Abwärmerückgewinnung in der Stahlproduktion. Ein \ac{milp} Modell wurde verwendet, um Betriebspläne zu erstellen. Die experimentelle Validierung an einer Testanlage zeigte vielversprechende Ergebnisse. Jedoch wurden die Tests in einer Laborumgebung durchgeführt, und weitere methodische Verbesserungen sind notwendig, um die Ansätze auf industrielle Anwendungen zu übertragen. Langzeituntersuchungen und umfassendere Tests in industriellen Umgebungen fehlen.


\citet{BHA+23} untersuchen die  Optimierung des Betriebs von Wärmepumpen. \citet{KSB+24} implementieren einen Optimierungsansatz zur Abwärmerückgewinnung in der Stahlproduktion. Beide Arbeiten stellen Tests der jeweiligen Ansätze in einer Laborumgebung vor. Eine weiterführende Anwendung unter realen Betriebsbedingungen wird jedoch nicht beschrieben, um die Ergebnisse umfassend zu validieren.


%### 4. "Quantifying the Demand Response Potential of Inherent Energy Storages in Production Systems" von Strobel et al.

\todo[inline]{\citet{SFW+20} weiter analysieren}
\citet{SFW+20} entwickeln ein Modell zur Bewertung des Flexibilitätspotenzials von inhärenten Energiespeichern in Produktionssystemen und testen es an einer Produktionslinie der Metallbearbeitungsindustrie. Das Modell ermöglicht die Echtzeitüberwachung und Nutzung des Flexibilitätspotenzials zur Netzstabilisierung. Obwohl das Modell in einer realen Produktionsumgebung angewendet wurde, stellt die Heterogenität der industriellen Maschinen und unzureichende Marktanreize eine Herausforderung dar. Langzeittests und Validierungen in verschiedenen industriellen Umgebungen fehlen, um die Generalisierbarkeit und langfristige Effizienz der Ansätze zu bestätigen.
\todo[inline]{Ich hab es gerade wirklich nur kurz überfolgen, aber Quantifizieren die nicht nur Flexibilität? Habe nicht gesehen, dass die Anlagen auch flexibel betrieben werden.  }


Die Analyse verwandter Arbeiten zeigt, dass obwohl Modelle und Ansätze zur Optimierung des Energieverbrauchs einer Vielzahl von Anlagen präsentiert werden, es nur eine begrenzte Anzahl an Arbeiten gibt, die diese Modelle unter realen Betriebsbedingungen validieren. Ebenfalls wird meist nicht der Einfluss der Veränderung des Energieverbrauchs auf die Produktionsmenge der Anlage betrachtet \cite{GFS+22}. Die praktische Implementierung und Auswirkungen in industriellen Umgebungen bleiben daher oft ungetestet.

==> acronyms.tex <==
%alphabetisch anordnen
%https://www.namsu.de/Extra/pakete/Acronym.html
% Beispiel: \acro{1}[2]{3}
% 1: so wird die Abkürzung im Text mit \ac{1} aufgerufen. 
% beim ersten Aufruf steht dann da 3 (2), also
% 2: richtige Schreibweise der Abkürzung
% 3: Langform der Abkürzung
% -- A ------------------------------------------------------------------------------------------------------%
% -- B ------------------------------------------------------------------------------------------------------%
\acro{BESS}{Battery energy storage system}
\acrodefplural{BESS}[BESS]{Battery energy storage systems}
\acro{bdew}[BDEW]{Bundesverband der Energie- und Wasserwirtschaft}
% -- C ------------------------------------------------------------------------------------------------------%
\acro{CHP}{Combined heat and power}
\acro{co2}[CO$_2$]{Kohlenstoffdioxid}
% -- D ------------------------------------------------------------------------------------------------------%
% -- E ------------------------------------------------------------------------------------------------------%
\acro{EEG}{Erneuerbare Energien Gesetz}
\acro{EU}{Europäische Union}
\acro{EV}{Electric vehicle}
\acrodefplural{EV}[EVs]{Electric vehicles}
% -- F ------------------------------------------------------------------------------------------------------%
% -- G ------------------------------------------------------------------------------------------------------%
% -- H ------------------------------------------------------------------------------------------------------%
\acro{HVAC}{Heating, Ventilation, and Air Conditioning}
% -- I ------------------------------------------------------------------------------------------------------%
% -- J ------------------------------------------------------------------------------------------------------%
% -- K ------------------------------------------------------------------------------------------------------%
% -- L ------------------------------------------------------------------------------------------------------%
\acro{LoD}{Level of Detail}
\acro{LP}{Linear programming}
% -- M ------------------------------------------------------------------------------------------------------%
\acro{MH}{Meta heuristic}
\acro{MPC}{Model-predictive control}
% -- N ------------------------------------------------------------------------------------------------------%
 \acro{NLP}{Non-linear programming}
% -- O ------------------------------------------------------------------------------------------------------%
% -- P ------------------------------------------------------------------------------------------------------%
\acro{PV}{Photovolatik}
% -- Q ------------------------------------------------------------------------------------------------------%
%\acro{QP}{Quadratic programming}
% -- R ------------------------------------------------------------------------------------------------------%
% -- S ------------------------------------------------------------------------------------------------------%
\acro{SOC}{Speicherzustand, eng. \emph{State of Charge}}
\acro{SP}{Stochastic programming}
% -- T ------------------------------------------------------------------------------------------------------%
\acro{TCL}{Thermostatically controlled loads}
% -- U ------------------------------------------------------------------------------------------------------%
% -- V ------------------------------------------------------------------------------------------------------%
% \acro{VRE}{Variable renewable energy}
\acro{VPP}{Virtual power plant}
% -- W ------------------------------------------------------------------------------------------------------%
% -- X ------------------------------------------------------------------------------------------------------%
% -- Y ------------------------------------------------------------------------------------------------------%
% -- Z ------------------------------------------------------------------------------------------------------%

